Relaxed Clustered Hawkes Process for Procrastination Modeling in MOOCs

Hawkes processes have been shown to be efficient in modeling bursty sequences in a variety of applications, such as finance and social network activity analysis. Traditionally, these models parameterize each process independently and assume that the history of each point process can be fully observed. Such models could however be inefficient or even prohibited in certain real-world applications, such as in the field of education, where such assumptions are violated. Motivated by the problem of detecting and predicting student procrastination in students Massive Open Online Courses (MOOCs) with missing and partially observed data, in this work, we propose a novel personalized Hawkes process model (RCHawkes-Gamma) that discovers meaningful student behavior clusters by jointly learning all partially observed processes simultaneously, without relying on auxiliary features. Our experiments on both synthetic and real-world education datasets show that RCHawkes-Gamma can effectively recover student clusters and their temporal procrastination dynamics, resulting in better predictive performance of future student activities. Our further analyses of the learned parameters and their association with student delays show that the discovered student clusters unveil meaningful representations of various procrastination behaviors in students.

==> metrics.tex <==
Our experiment setup represents a real-world scenario, in which some student activity data are missing because a student missed an assignment, they have not completed their activities on an assignment (missing past assignment), or have not started the assignment yet (unseen future assignment).
% It is also common to use activity records of students in previous offerings of a course in conjunction with the new semester students' activities for learning analytics.
% Thus, it is likely to have all students' activities before a specific time $T$, by which some students' activities on part of the assignments are missing.
% We are interested in predicting these students' \textit{future} possible activities. 

To replicate this scenario in the simulated data, we randomly select a ratio $r$ of students and set their activities for the last two assignments to be completely missing (\textit{unseen} future assignment). As a result, in total, we have $r\times 90\times 2$ assignment-student pairs' activities to be completely unseen. In the rest of the assignment-student pairs that do have past activities, for each of them
% For the rest of the students, for each of their activity sequences on all assignments, 
we keep the earliest $70\%$ of activity occurrences as training and the rest $30\%$ of them to be testing (assignments with \textit{seen} history).
An illustration of this setting is shown in Fig.~\ref{fig:illu_data}. Each cell represents an assignment-user pair, and the orange area represents the first $70\%$ of the observed time stamps used for training, blue area represents the rest of $30\%$ used for testing and the grey area represents the assignment-user pairs that are held out to simulate the scenario when the history is totally unseen.

\begin{figure}
    \centering
    \includegraphics[width =0.7 \linewidth]{figs/illustration_split3.png}
    \caption{Illustration of unseen, train and test splits of data in experiment setup.}
    \label{fig:illu_data}
    \vspace{-10pt}
\end{figure}
%In the experiments on synthetic data, we select a ratio $r$ of students and hold out all of their activities on the last two assignments.
%For the rest of the processes, we use the earliest $70\%$ of activity occurrences as training and the rest $30\%$ of them to be testing (in a real-world scenario, students might revisit or resubmit a past assignment at any point during the course until the assignment is locked), where $r$ represents the portion of the processes that are unseen. 
In real datasets, the unit time is set to be an hour for all observed assignment student pairs in both courses. 
We use the timestamps of the activities that took place before the midpoint of the last assignment (from when it was published until it was locked) as training. 
Hyper parameters $k$, $\beta$ and penalty coefficients are selected using grid search. 


%Last but not least, because our model captures the cluster structure of parameter matrix $A$, we also compare the correlation matrix of $\hat{A}$ estimated by each model. 


==> related.tex <==
%---------------------------------------- bacground material

\subsection{Low-Rank Hawkes Processes}
\label{sec:related:hawkes}
Hawkes processes~\cite{Hawkes1971} have been successfully used to model processes in applications, such as social networks%~\cite{Zhou2013,Linderman2014,Zhao2015, Farajtabar2017,
~\cite{Chen2019}, mobility patterns~\cite{Vassoy2019}, %,Wang2017,Vassoy2019},Du2016 
and recommender systems~\cite{Du2015,Jing2017}. %Xiao2016.
%For example, Du et al. proposed a topic-sensitive information diffusion model in social networks based on multivariate Hawkes processes to estimate the topic-dependent transmission rates~\cite{Du2013}.
%However, their application in the field of Educational Data Mining is limited.
%\noindent\textbf{Low-Rank Hawkes Processes}
Among them, the most relevant work to our paper is a low-rank uni-variate Hawkes process proposed by Du et al., to capture user-item interaction and recommending items ``at the right moment''~\cite{Du2015}. 
%Their experiments include recommending items to users according to a ranked list of estimated item intensities for each user and predicting the returning time for an interaction between a user and an item by average sampling from the density of the next event time, both evaluated by mean absolute error.
However, this work does not incorporate the clustering behavior that is essential in our problem domain.
We include this model as one of our baselines.
%The most relevant literature on Hawkes processes to our work is low-rank or structured Hawkes processes inspired by reducing the number of learned parameters~\cite{Zhou2013,Du2015,Shang2019}.
%Other than the work by Du et al.~\cite{Du2015}, 
% Other relevant literature on Hawkes processes % either 
% \textcolor{orange}{either mainly focus on modeling mutual excitation among sequences, i.e. multi-variate Hawkes processes~\cite{liu2018exploiting}}, or require auxiliary information in addition to the event sequences \textcolor{orange}{~\cite{li2020tweedie}}
% For others that do not necessarily require auxiliary information, they are not capable of inferring future activity arrival time of unobserved samples. It is because, in traditional Hawkes models, all sequences are usually learned independently and no relatedness among the processes are assumed. Whereas in more recent RNN-based models, the prediction of future is computed conditioning on the past observations, thus historical observations are crucial for meaningful predictions (\cite{du2016recurrent, xiao2017modeling}.
%to our work are low-rank or structured multidimensional Hawkes processes and low-rank Hawkes processes with auxiliary information. %inspired by reducing the number of learned parameters~\cite{Zhou2013,Du2015,Shang2019}, 
%In the following, we will briefly go over these relevant literature and the process mining literature with applications in education.


%\noindent\textbf{Low-Rank Multi-Dimensional Hawkes Processes.}
%Most of the current work in low-rank Hawkes processes are modeling multi-dimensional Hawkes processes. 
Unlike uni-variate Hawkes, Multi-variate Hawkes processes assume that there are multiple types of sequences with mutual excitement between them~\cite{Zhou2013,Luo2015,Bacry2015,Lemonnier2017}.
In other words, they assume a triggering effect between different sequences of process types.
For example, in modeling news propagation trends across different social networks, such as twitter and Facebook, one can assume that, an activity in one social network (e.g., a tweet in twitter) can trigger an activity in another social network (e.g., a post in Facebook).
Even though the low-rank assumption has been used in some multi-variate Hawkes models~\cite{Zhou2013,bompaire2020sparse}, this assumption is usually imposed based on the similarities between activity types, rather than between time sequences of different users or user-item pairs.
% Zhou et al. propose a low-rank multidimensional Hawkes process, in social setting, using both low-rank and sparse regularizations on intensity parameter matrix~\cite{Zhou2013};
%Luo et al. propose a multi-task multidimensional Hawkes process model that captures the structures between sequences of multiple activity types by imposing both nuclear-rank and L1-rank constraints~\cite{Luo2015}; and
%As an example of these works, Lemonnier et al. propose to use matrix decomposition on the intensity matrix for multivariate Hawkes processes for the purpose of having a more computationally efficient learning algorithm for large-scale datasets with many dimensions~\cite{Lemonnier2017}.
%To strengthen the theory behind low-rank constraints on multivariate Hawkes processes, Bacry et al. have studied and drawn error bounds for various combinations of L1 and nuclear norm regularizations and concluded that the weighted L1 penalization of intensity and burstiness parameters and with or without the trace-norm penalization of burstiness leads to a better recovery of original data parameters~\cite{Bacry2015}.
%As a result, sequences in different social networks can be modeled by different process types, that in addition to within-type self-excitements, can trigger sequences of other process types.
Furthermore, in our application of modeling students' procrastination behavior, neither a students' activity triggers another student's activity, nor the deadline of one assignment triggers the activities that are related to another assignment.
Since the assignments are not parallel, activities for each assignment are only triggered by the same assignment's deadline.
Also, since students do not work in teams and are not in a social setting, studying activities of each student can only be the offspring of the same student's past activities.
Hence, we build our model based on the uni-variate Hawkes process.


%\noindent\textbf{Low-Rank Uni-Variate Hawkes Processes with Auxiliary Information.}
\textcolor{blue}{Some other recent works model low-rank uni-variate Hawkes processes, in presence of auxiliary information~\cite{He2015,Du2015a,Li2018,Shang2018,shang2019geometric}}.
%For example, in the recommender system setting, Shang et al. impose a local low-rank constraint on intensity parameter matrix to model large-scale user-item interactions.
%Their model requires auxiliary information, such as item features, that capture the similarity between user-item pairs~\cite{Shang2018}.
%They recommend items to users according to a ranked list of estimated survivals for items at time $t$ (evaluated by mean average rank) and estimate the interaction time by calculating the expected value of the (intensity $\times$ survival) at time $t$ (evaluated by mean absolute error).
%Later, they propose geometric Hawkes process~\cite{Shang2019} that incorporates the Laplacian of an input graph. 
For example, in the recommender system setting, Shang et al.~\cite{shang2019geometric} propose geometric Hawkes process that requires an input graph to constraint the burstiness and intensity parameters. 
%geometric deep learning as a representation of proximity networks, by using their parameters in the Hawkes objective function and adding observed graph Laplacian constraints to find burstiness and intensity parameters.
As another example, for the problem of clustering document streams, Du et al. propose a Dirichlet-Hawkes process model that uses document content as auxiliary information to learn topic clusters~\cite{Du2015a}. % while learning topic clusters for documents according to their content, adjusts their preferential attachment to the clusters according to the learned Hawkes intensity of the cluster topics~\cite{Du2015a}.
Conversely, due to privacy constraints in our application, many educational datasets are highly anonymized and there is a scarcity of auxiliary information in them.
Consequently, having a model that does not require such information is valuable in our context.



%multi-variate Hawkes with external information and text clustering  

%Note that in this model the graph Laplacians are given, and are not estimated by the model.

% They learn one set of inter-dimension triggering effect parameters per-user, vectorize it, and impose the low-rank constraints on a concatenation of these parameters. (for all users) They assume that assignments are not independent and are triggering each other, but users can be clustered according to their multi-variate A matrices.


% why we're not using multi-dimensional hawkes


% The most relevant to us:




% hawkes clustering/text 


% some less related work:
%

% \noindent\textbf{Hawkes Processes in Educational Data Mining.}
% In the educational domain, a few works has used Hawkes processes, especially to model social and interaction data among students~\cite{Halpin2013,Halpin2017,Lan2018}.
% For example, Von Davier has suggested using Hawkes processes in modeling the collaboration dynamics between students within and between groups~\cite{Davier2013};
% Halpin et al. used multi-dimensional Hawkes processes to measure students' engagement in collaborating with each other~\cite{Halpin2013,Halpin2017}; and
% Lan et al. modeled students' posting and replying activities in a MOOC's discussion forum to recommend useful discussion threads to students~\cite{Lan2018}.
% Another interesting application of Hawkes process in the education domain is the work by Boerner et al. that analyzes the association between student skills and skills required by professional jobs~\cite{Boerner2018}.
% In another recent work, Cai et al. proposed to use long and short multi-dimensional Hawkes processes to discover the associations between different types of learning activities in MOOCs, according to all activities of the general student population, without modeling individual students~\cite{Cai2018}.
% None of the above research uses Hawkes processes to model the procrastination behavior, nor considers course deadlines and milestones in their application of Hawkes process.
% \color{red}
% To the best of our knowledge, the only work that uses Hawkes processes to model student procrastination behavior is by Yao et al.~\cite{Yao2020} which is not low-rank, does not model student behavior clusters, and cannot infer unseen data.
% We include this model in our experiments as one of our baselines.
% \color{black}

% ~\cite{Pang2018} weird! not learning hawkes params, but just uses the formulation with some predefined params.
% ~\cite{Ejima2019} engagement in general, not ed
% ~\cite{Shchur2019,Mozer2017} archive. predicting student interaction time with a MOOC system~\cite{Shchur2019} (also ICLR 2020).
% ~\cite{Davier2013} just proposes to use Hawkes.

\subsection{Procrastination Modeling in Education Domain.}
As there is no quantitative definition for procrastination behavior, in most of the recent educational data mining literature, procrastination-related behavior has been summarized by curating time-related features from student interactions in the course.
These studies aim to evaluate the relationship between these time-related features with student performance and do not model temporal aspects of procrastination~\cite{Baker2016,Cerezo2017,Kazerouni2017}.
The few recent work that model student activity sequences, are limited in their assumptions, do not capture student activity intensities, are not personalized, do not model time dependencies between student actions, and do not infer missing data~\cite{Park2018,Yao2020}. 
%Capturing the temporal aspects of procrastination, such as activity intensity or burstiness, has been attempted in a few numbers of recent works~\cite{Backhage2017,Park2018}.

As an example, Park et al. classify students to procrastinators vs. non-procrastinators by formulating a measure using a mixture model of per-day student activity counts during each week of the course~\cite{Park2018}.
Even though each student's activity is counted in a daily basis, it is not a temporal approach that models activity time points. Instead, it assumes that students' activities \textit{counts} can be modeled by a mixture Poisson distribution, thus they are able to compute the likelihood of students having more activities towards the end of the week or not. As a result, it cannot predict \textit{when} future activities will happen. Furthermore, it also cannot capture non-homogeneously spaced deadlines in a course.
% Similarly, Backhage et al. proposed Poisson distribution to model students' daily activity count in order to capture procrastination-deadline cycles of all students in the course~\cite{Backhage2017}. % dynamics of student population interaction with online courses 
However, this model assumes that all students follow the same procrastination behavior during the course and does not distinguish the differences between student behaviors.
% In their work, each day of the week is associated with a Poisson rate parameter that is constant during the whole course.
% Despite representing individual student activity counts, this model cannot differentiate between different weeks in the course, does not have a continuous time scale, and cannot capture non-homogeneously spaced deadlines in a course.

To the best of our knowledge, the only work that uses Hawkes processes to model student procrastination behavior is by Yao et al.~\cite{Yao2020} that uses activity types as auxiliary information, to model student procrastination behavior.
This model is not low-rank, does not model student behavior clusters, and cannot infer unseen data.
Since this model is the closest research on procrastination modeling to our work,
we include this model in our experiments as one of our baselines, even though it uses a multi-variate Hawkes model.
\color{black}

